On inversion sets and the weak order in Coxeter groups

In this article, we investigate the existence of joins in the weak order of an infinite Coxeter group W. We give a geometric characterization of the existence of a join for a subset X in W in terms of the inversion sets of its elements and their position relative to the imaginary cone. Finally, we discuss inversion sets of infinite reduced words and the notions of biconvex and biclosed sets of positive roots.

==> Fig6.tex <==
\begin{tikzpicture}
	[scale=2,
	 q/.style={red,line join=round,thick},
	 racine/.style={blue},
	 racinesimple/.style={inner sep=2pt,circle,draw=blue!75!black,fill=blue!40,thick},
	 racinedih/.style={blue},
	 rotate=0]


\def\grosseur{0.025}
\def\grosseursimple{0.05}

\def\grosseurdih{0.0075}

\fill[red] (2.00000000000000,1.15470053837925) circle (\grosseursimple);

\fill[red, fill opacity=0.5] (0.000000000000000,0.000000000000000) -- (2,0) -- (2.00000000000000,1.15470053837925) -- cycle;
\fill[cyan, fill opacity=0.5] (4,0) -- (2,0) -- (2.00000000000000,1.15470053837925) -- cycle;

% Roots of deepness= 1
\node[racinesimple, label=left :{$\alpha$}] (a) at (0,0) {};
\node[racinesimple, label=right :{$\beta$}] (b) at (4,0) {};
\node[racinesimple, label=above:{$\gamma$}] (g) at (2.00000000000000,3.46410161513775) {};
\draw[green!75!black] (a) -- (b) -- (g) -- (a);
% Roots of deepness= 2
\fill[racine] (3.00000000000000,1.73205080756888) circle (\grosseur);
\fill[racine] (2.00000000000000,0.01) circle (\grosseur);
\fill[racine] (1.00000000000000,1.73205080756888) circle (\grosseur);

% Roots of deepness= 3
\fill[racine] (2.50000000000000,0.866025403784439) circle (\grosseur);
\fill[racine] (1.50000000000000,0.866025403784439) circle (\grosseur);
\fill[racine] (2.00000000000000,1.73205080756888) circle (\grosseur);

% Roots of deepness= 4
\fill[racine] (2.00000000000000,0.692820323027551) circle (\grosseur);
\fill[racine] (2.40000000000000,1.38564064605510) circle (\grosseur);
\fill[racine] (1.60000000000000,1.38564064605510) circle (\grosseur);

% Roots of deepness= 5
\fill[racine] (1.71428571428571,0.989743318610787) circle (\grosseur);
\fill[racine] (2.28571428571429,0.989743318610787) circle (\grosseur);
\fill[racine] (2.00000000000000,1.48461497791618) circle (\grosseur);

% Roots of deepness= 6
\fill[racine] (1.75000000000000,1.29903810567666) circle (\grosseur);
\fill[racine] (2.25000000000000,1.29903810567666) circle (\grosseur);
\fill[racine] (2.00000000000000,0.866025403784439) circle (\grosseur);

% Roots of deepness= 7
\fill[racine] (2.20000000000000,1.03923048454133) circle (\grosseur);
\fill[racine] (1.80000000000000,1.03923048454133) circle (\grosseur);
\fill[racine] (2.00000000000000,1.38564064605510) circle (\grosseur);

% Roots of deepness= 8
\fill[racine] (1.81818181818182,1.25967331459555) circle (\grosseur);
\fill[racine] (2.18181818181818,1.25967331459555) circle (\grosseur);
\fill[racine] (2.00000000000000,0.944754985946660) circle (\grosseur);

% Roots of deepness= 9
\fill[racine] (2.00000000000000,1.33234677505298) circle (\grosseur);
\fill[racine] (1.84615384615385,1.06587742004239) circle (\grosseur);
\fill[racine] (2.15384615384615,1.06587742004239) circle (\grosseur);

% Roots of deepness= 10
\fill[racine] (1.85714285714286,1.23717914826348) circle (\grosseur);
\fill[racine] (2.00000000000000,0.989743318610787) circle (\grosseur);
\fill[racine] (2.14285714285714,1.23717914826348) circle (\grosseur);

%\coordinate (ancre) at (-0.5,2.6);
%\node[sommet,label=below left:$s_\alpha$] (alpha) at (ancre) {};
%\node[sommet,label=below right :$s_\beta$] (beta) at ($(ancre)+(0.5,0)$) {} edge[thick] (alpha);
%\node[sommet,label=above:$s_\gamma$] (gamma) at ($(ancre)+(0.25,0.43)$) {} edge[thick] (alpha) edge[thick] (beta);
%\coordinate (mat) at (4, 2.8);
%\node at (mat) {$\left(\begin{array}{rrr}
%1 & -\frac{1}{2} & -\frac{1}{2} \\
%-\frac{1}{2} & 1 & -\frac{1}{2} \\
%-\frac{1}{2} & -\frac{1}{2} & 1
%\end{array}\right)$};

\node at ($(0,0)!0.5!(2,0)!0.33!(2,1.15470053837925)$) {A};
\node at ($(4,0)!0.5!(2,0)!0.33!(2,1.15470053837925)$) {B};

\node at (-0.5,1.5) {$N(\omega)=A\cap\Phi^+$};
\node at (4.5,1.5) {$N(\omega')=(A\cup B)\cap\Phi^+$};

\end{tikzpicture}


==> Fig7.tex <==
\begin{tikzpicture}
	[scale=2,
	 q/.style={red,line join=round,thick},
	 racine/.style={blue},
	 racinesimple/.style={black},
	 racinedih/.style={blue},
	 limit/.style={fill=red,draw=black,diamond},
	 limdir/.style={fill=orange,draw=black,diamond},
	 weight/.style={fill=green,draw=black,diamond},
	 sommet/.style={inner sep=2pt,circle,draw=black,fill=blue,thick,anchor=base},
	 rotate=0]


\def\grosseur{0.0125}
\def\grosseursimple{0.025}

\def\grosseurdih{0.0075}

%% La courbe Q

\draw[q] (3.15,1.24) -- (3.15,1.25) -- (3.14,1.33) -- (3.13,1.39) -- (3.12,1.43) -- (3.11,1.47) -- (3.10,1.50) -- (3.09,1.53) -- (3.08,1.56) -- (3.06,1.61) -- (3.05,1.63) -- (3.01,1.71) -- (3.00,1.73) -- (2.97,1.78) -- (2.95,1.81) -- (2.92,1.85) -- (2.89,1.89) -- (2.88,1.90) -- (2.75,2.03) -- (2.74,2.04) -- (2.69,2.08) -- (2.66,2.10) -- (2.63,2.12) -- (2.60,2.14) -- (2.55,2.17) -- (2.53,2.18) -- (2.51,2.19) -- (2.49,2.20) -- (2.44,2.22) -- (2.42,2.23) -- (2.39,2.24) -- (2.36,2.25) -- (2.33,2.26) -- (2.25,2.28) -- (2.21,2.29) -- (2.20,2.29) -- (2.14,2.30) -- (2.13,2.30) -- (1.87,2.30) -- (1.86,2.30) -- (1.80,2.29) -- (1.79,2.29) -- (1.75,2.28) -- (1.67,2.26) -- (1.64,2.25) -- (1.61,2.24) -- (1.58,2.23) -- (1.56,2.22) -- (1.51,2.20) -- (1.49,2.19) -- (1.47,2.18) -- (1.45,2.17) -- (1.40,2.14) -- (1.37,2.12) -- (1.34,2.10) -- (1.31,2.08) -- (1.26,2.04) -- (1.25,2.03) -- (1.12,1.90) -- (1.11,1.89) -- (1.08,1.85) -- (1.05,1.81) -- (1.03,1.78) -- (1.00,1.73) -- (0.990,1.71) -- (0.950,1.63) -- (0.940,1.61) -- (0.920,1.56) -- (0.910,1.53) -- (0.900,1.50) -- (0.890,1.47) -- (0.880,1.43) -- (0.870,1.39) -- (0.860,1.33) -- (0.850,1.25) -- (0.850,1.24) -- (0.850,1.07) -- (0.850,1.06) -- (0.860,0.980) -- (0.870,0.920) -- (0.880,0.880) -- (0.890,0.840) -- (0.900,0.810) -- (0.910,0.780) -- (0.920,0.750) -- (0.940,0.700) -- (1.00,0.580) -- (1.03,0.530) -- (1.05,0.500) -- (1.08,0.460) -- (1.11,0.420) -- (1.12,0.410) -- (1.26,0.270) -- (1.31,0.230) -- (1.40,0.170) -- (1.45,0.140) -- (1.47,0.130) -- (1.49,0.120) -- (1.51,0.110) -- (1.53,0.100) -- (1.58,0.0800) -- (1.61,0.0700) -- (1.67,0.0500) -- (1.70,0.0400) -- (1.74,0.0300) -- (1.79,0.0200) -- (1.85,0.0100) -- (1.86,0.0100) -- (2.14,0.0100) -- (2.15,0.0100) -- (2.21,0.0200) -- (2.26,0.0300) -- (2.30,0.0400) -- (2.33,0.0500) -- (2.39,0.0700) -- (2.42,0.0800) -- (2.47,0.100) -- (2.49,0.110) -- (2.51,0.120) -- (2.53,0.130) -- (2.55,0.140) -- (2.60,0.170) -- (2.69,0.230) -- (2.74,0.270) -- (2.88,0.410) -- (2.89,0.420) -- (2.92,0.460) -- (2.95,0.500) -- (2.97,0.530) -- (3.00,0.580) -- (3.06,0.700) -- (3.08,0.750) -- (3.09,0.780) -- (3.10,0.810) -- (3.11,0.840) -- (3.12,0.880) -- (3.13,0.920) -- (3.14,0.980) -- (3.15,1.06) -- (3.15,1.07) -- cycle;

% Roots of deepness= 0
\node[label=left :{$\alpha_r$}] (a) at (0.000000000000000,0.000000000000000) {};
\fill[racinesimple] (0.000000000000000,0.000000000000000) circle (\grosseursimple);
\node[label=right :{$\alpha_t$}] (b) at (4.00000000000000,0.000000000000000) {};
\fill[racinesimple] (4.00000000000000,0.000000000000000) circle (\grosseursimple);
\node[label=above :{$\alpha_s$}] (g) at (2.00000000000000,3.46410161513775) {};
\fill[racinesimple] (2.00000000000000,3.46410161513775) circle (\grosseursimple);

\draw[green!75!black] (a) -- (b) -- (g) -- (a);

% Roots of deepness= 1
\fill[racine] (1.33333333333333,2.30940107675850) circle (\grosseursimple);
\fill[racine] (1.33333333333333,0.01) circle (\grosseursimple);
\fill[racine] (0.666666666666667,1.15470053837925) circle (\grosseursimple);
\fill[racine] (2.66666666666667,2.30940107675850) circle (\grosseursimple);
\fill[racine] (3.33333333333333,1.15470053837925) circle (\grosseursimple);
\fill[racine] (2.66666666666667,0.01) circle (\grosseursimple);

% Roots of deepness= 2
\fill[racine] (0.800000000000000,1.38564064605510) circle (\grosseursimple);
\fill[racine] (1.60000000000000,0.01) circle (\grosseursimple);
\fill[racine] (1.20000000000000,2.07846096908265) circle (\grosseursimple);
\fill[racine] (2.80000000000000,2.07846096908265) circle (\grosseursimple);
\fill[racine] (0.888888888888889,0.769800358919501) circle (\grosseur);
\fill[racine] (2.88888888888889,0.384900179459750) circle (\grosseur);
\fill[racine] (2.22222222222222,2.30940107675850) circle (\grosseur);
\fill[racine] (2.40000000000000,0.01) circle (\grosseursimple);
\fill[racine] (3.11111111111111,0.769800358919501) circle (\grosseur);
\fill[racine] (1.77777777777778,2.30940107675850) circle (\grosseur);
\fill[racine] (1.11111111111111,0.384900179459750) circle (\grosseur);
\fill[racine] (3.20000000000000,1.38564064605510) circle (\grosseursimple);

\draw (1.33333333333333,2.30940107675850) -- (2.66666666666667,2.30940107675850);

\node[label=left :{$s(\alpha_r)$}] (b) at (1.33333333333333,2.30940107675850) {};
\node[label=right :{$s(\alpha_t)$}] (b) at (2.66666666666667,2.30940107675850) {};

\draw (1.33333333333333,2.30940107675850) -- (4,0);

\node[label=right :{$t s(\alpha_r)$}] (b) at (3.11111111111111,0.769800358919501) {};

\end{tikzpicture}
